Tales of Tension: Magnetized Infalling Clouds and Cold Streams in the CGM

The observed star formation and wind outflow rates in galaxies suggest cold gas must be continually replenished via infalling clouds or streams. Previous studies have highlighted the importance of cooling-induced condensation on such gas, which enables survival, mass growth, and a drag force which typically exceeds hydrodynamic drag. However, the combined effects of magnetic fields, cooling, and infall remains unexplored. We conduct 3D magnetohydrodynamic (MHD) simulations of radiatively cooling infalling clouds and streams in uniform and stratified backgrounds. For infalling clouds, magnetic fields aligned with gravity do not impact cloud growth or dynamics significantly, although we see enhanced survival for stronger fields. By contrast, even weak transverse magnetic fields significantly slow cloud infall via magnetic drag, due to the development of strong draped fields which develop at peak infall velocity, before the cloud decelerates. Besides enhancing survival, long, slow infall increases total cloud mass growth compared to the hydrodynamic case, even if reduced turbulent mixing lowers the rate of mass growth. Streams often result in qualitatively different behavior. Mass growth and hence accretion drag are generally much lower in hydrodynamic streams. Unlike in clouds, aligned magnetic fields suppress mixing and thus both mass growth or loss. Transverse fields do apply magnetic drag and allow streams to grow, when the streams have a well-defined 'head' pushing through the surrounding medium. Overall, regardless of the efficacy of drag forces, streams are surprisingly robust in realistic potentials, as the destruction time when falling supersonically exceeds the infall time. We develop analytic models which reproduce cloud/stream trajectories.

==> main <==
\begin{thebibliography}{}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\url}[1]{\href{#1}{#1}}
\providecommand{\dodoi}[1]{doi:~\href{http://doi.org/#1}{\nolinkurl{#1}}}
\providecommand{\doeprint}[1]{\href{http://ascl.net/#1}{\nolinkurl{http://ascl.net/#1}}}
\providecommand{\doarXiv}[1]{\href{https://arxiv.org/abs/#1}{\nolinkurl{https://arxiv.org/abs/#1}}}

\bibitem[{{Abruzzo} {et~al.}(2022){Abruzzo}, {Bryan}, \&
  {Fielding}}]{Abruzzo2022}
{Abruzzo}, M.~W., {Bryan}, G.~L., \& {Fielding}, D.~B. 2022, \apj, 925, 199,
  \dodoi{10.3847/1538-4357/ac3c48}

\bibitem[{{Antolin} \& {Rouppe van der Voort}(2012)}]{antolin2012}
{Antolin}, P., \& {Rouppe van der Voort}, L. 2012, \apj, 745, 152,
  \dodoi{10.1088/0004-637X/745/2/152}

\bibitem[{{Antolin} {et~al.}(2010){Antolin}, {Shibata}, \&
  {Vissers}}]{antolin2010}
{Antolin}, P., {Shibata}, K., \& {Vissers}, G. 2010, \apj, 716, 154,
  \dodoi{10.1088/0004-637X/716/1/154}

\bibitem[{{Aung} {et~al.}(2024){Aung}, {Mandelker}, {Dekel}, {Nagai},
  {Semenov}, \& {van den Bosch}}]{Aung2024}
{Aung}, H., {Mandelker}, N., {Dekel}, A., {et~al.} 2024, arXiv e-prints,
  arXiv:2403.00912, \dodoi{10.48550/arXiv.2403.00912}

\bibitem[{{Aung} {et~al.}(2019){Aung}, {Mandelker}, {Nagai}, {Dekel}, \&
  {Birnboim}}]{Aung2019}
{Aung}, H., {Mandelker}, N., {Nagai}, D., {Dekel}, A., \& {Birnboim}, Y. 2019,
  \mnras, 490, 181, \dodoi{10.1093/mnras/stz1964}

\bibitem[{{Begelman} \& {Fabian}(1990)}]{Begelman1990}
{Begelman}, M.~C., \& {Fabian}, A.~C. 1990, \mnras, 244, 26P

\bibitem[{{Benjamin} \& {Danly}(1997)}]{BenjaminDanly}
{Benjamin}, R.~A., \& {Danly}, L. 1997, \apj, 481, 764, \dodoi{10.1086/304078}

\bibitem[{{Berlok} \& {Pfrommer}(2019)}]{BerlokColdStream}
{Berlok}, T., \& {Pfrommer}, C. 2019, \mnras, 489, 3368,
  \dodoi{10.1093/mnras/stz2347}

\bibitem[{{Bouch{\'e}} {et~al.}(2016){Bouch{\'e}}, {Finley}, {Schroetter},
  {Murphy}, {Richter}, {Bacon}, {Contini}, {Richard}, {Wendt}, {Kamann},
  {Epinat}, {Cantalupo}, {Straka}, {Schaye}, {Martin}, {P{\'e}roux},
  {Wisotzki}, {Soto}, {Lilly}, {Carollo}, {Brinchmann}, \&
  {Kollatschny}}]{Bouche2016}
{Bouch{\'e}}, N., {Finley}, H., {Schroetter}, I., {et~al.} 2016, \apj, 820,
  121, \dodoi{10.3847/0004-637X/820/2/121}

\bibitem[{{Braun} \& {Burton}(1999)}]{braun99}
{Braun}, R., \& {Burton}, W.~B. 1999, \aap, 341, 437,
  \dodoi{10.48550/arXiv.astro-ph/9810433}

\bibitem[{{Breitschwerdt} {et~al.}(1991){Breitschwerdt}, {McKenzie}, \&
  {Voelk}}]{breitschwerdt91}
{Breitschwerdt}, D., {McKenzie}, J.~F., \& {Voelk}, H.~J. 1991, \aap, 245, 79

\bibitem[{{Cantalupo} {et~al.}(2014){Cantalupo}, {Arrigoni-Battaia},
  {Prochaska}, {Hennawi}, \& {Madau}}]{Cantalupo2014}
{Cantalupo}, S., {Arrigoni-Battaia}, F., {Prochaska}, J.~X., {Hennawi}, J.~F.,
  \& {Madau}, P. 2014, \nat, 506, 63, \dodoi{10.1038/nature12898}

\bibitem[{{Churazov} {et~al.}(2003){Churazov}, {Forman}, {Jones}, \&
  {B{\"o}hringer}}]{Churazov2003}
{Churazov}, E., {Forman}, W., {Jones}, C., \& {B{\"o}hringer}, H. 2003, \apj,
  590, 225, \dodoi{10.1086/374923}

\bibitem[{{Cottle} {et~al.}(2020){Cottle}, {Scannapieco}, {Br{\"u}ggen},
  {Banda-Barrag{\'a}n}, \& {Federrath}}]{Cottle2020}
{Cottle}, J., {Scannapieco}, E., {Br{\"u}ggen}, M., {Banda-Barrag{\'a}n}, W.,
  \& {Federrath}, C. 2020, \apj, 892, 59, \dodoi{10.3847/1538-4357/ab76d1}

\bibitem[{{{\c{S}}ahin} {et~al.}(2023){{\c{S}}ahin}, {Antolin}, {Froment}, \&
  {Schad}}]{sahin2023}
{{\c{S}}ahin}, S., {Antolin}, P., {Froment}, C., \& {Schad}, T.~A. 2023, \apj,
  950, 171, \dodoi{10.3847/1538-4357/acd44b}

\bibitem[{{Daddi} {et~al.}(2021){Daddi}, {Valentino}, {Rich}, {Neill},
  {Gronke}, {O'Sullivan}, {Elbaz}, {Bournaud}, {Finoguenov}, {Marchal},
  {Delvecchio}, {Jin}, {Liu}, {Strazzullo}, {Calabro}, {Coogan}, {D'Eugenio},
  {Gobat}, {Kalita}, {Laursen}, {Martin}, {Puglisi}, {Schinnerer}, \&
  {Wang}}]{Daddi2021}
{Daddi}, E., {Valentino}, F., {Rich}, R.~M., {et~al.} 2021, \aap, 649, A78,
  \dodoi{10.1051/0004-6361/202038700}

\bibitem[{{Das} \& {Gronke}(2023)}]{das23}
{Das}, H.~K., \& {Gronke}, M. 2023, \mnras, \dodoi{10.1093/mnras/stad3125}

\bibitem[{{de Boor}(1972)}]{DEBOOR197250}
{de Boor}, C. 1972, Journal of Approximation Theory, 6, 50,
  \dodoi{https://doi.org/10.1016/0021-9045(72)90080-9}

\bibitem[{{Dekel} \& {Birnboim}(2006)}]{DekelBrinboim2006}
{Dekel}, A., \& {Birnboim}, Y. 2006, \mnras, 368, 2,
  \dodoi{10.1111/j.1365-2966.2006.10145.x}

\bibitem[{{Dekel} {et~al.}(2013){Dekel}, {Zolotov}, {Tweed}, {Cacciato},
  {Ceverino}, \& {Primack}}]{dekel2013}
{Dekel}, A., {Zolotov}, A., {Tweed}, D., {et~al.} 2013, \mnras, 435, 999,
  \dodoi{10.1093/mnras/stt1338}

\bibitem[{{Dekel} {et~al.}(2009){Dekel}, {Birnboim}, {Engel}, {Freundlich},
  {Goerdt}, {Mumcuoglu}, {Neistein}, {Pichon}, {Teyssier}, \&
  {Zinger}}]{dekel09}
{Dekel}, A., {Birnboim}, Y., {Engel}, G., {et~al.} 2009, \nat, 457, 451,
  \dodoi{10.1038/nature07648}

\bibitem[{Dimotakis(1991)}]{dimotakis}
Dimotakis, P.~E. 1991, Tech. rep., Turbulent Free Shear Layer Mixing and
  Combustion

\bibitem[{{Dursi} \& {Pfrommer}(2008)}]{dursi08}
{Dursi}, L.~J., \& {Pfrommer}, C. 2008, \apj, 677, 993, \dodoi{10.1086/529371}

\bibitem[{{Emonts} {et~al.}(2023){Emonts}, {Lehnert}, {Yoon}, {Mandelker},
  {Villar-Mart{\'\i}n}, {Miley}, {De Breuck}, {P{\'e}rez-Torres}, {Hatch}, \&
  {Guillard}}]{EmontsColdStream}
{Emonts}, B. H.~C., {Lehnert}, M.~D., {Yoon}, I., {et~al.} 2023, Science, 379,
  1323, \dodoi{10.1126/science.abh2150}

\bibitem[{{Erb}(2008)}]{erb08}
{Erb}, D.~K. 2008, \apj, 674, 151, \dodoi{10.1086/524727}

\bibitem[{{Faucher-Giguere} \& {Oh}(2023)}]{CGMReviewPeng}
{Faucher-Giguere}, C.-A., \& {Oh}, S.~P. 2023, arXiv e-prints,
  arXiv:2301.10253, \dodoi{10.48550/arXiv.2301.10253}

\bibitem[{{Fielding} \& {Bryan}(2022)}]{FieldingBryanWinds}
{Fielding}, D.~B., \& {Bryan}, G.~L. 2022, \apj, 924, 82,
  \dodoi{10.3847/1538-4357/ac2f41}

\bibitem[{{Fielding} {et~al.}(2020){Fielding}, {Ostriker}, {Bryan}, \&
  {Jermyn}}]{fielding20}
{Fielding}, D.~B., {Ostriker}, E.~C., {Bryan}, G.~L., \& {Jermyn}, A.~S. 2020,
  arXiv e-prints, arXiv:2003.08390.
\newblock \doarXiv{2003.08390}

\bibitem[{{Fu} {et~al.}(2021){Fu}, {Xue}, {Prochaska}, {Stockton}, {Ponnada},
  {Lau}, {Cooray}, \& {Narayanan}}]{Fu2021}
{Fu}, H., {Xue}, R., {Prochaska}, J.~X., {et~al.} 2021, \apj, 908, 188,
  \dodoi{10.3847/1538-4357/abdb32}

\bibitem[{{Fumagalli} {et~al.}(2017){Fumagalli}, {Mackenzie}, {Trayford},
  {Theuns}, {Cantalupo}, {Christensen}, {Fynbo}, {M{\o}ller}, {O'Meara},
  {Prochaska}, {Rafelski}, \& {Shanks}}]{Fumagalli2017}
{Fumagalli}, M., {Mackenzie}, R., {Trayford}, J., {et~al.} 2017, \mnras, 471,
  3686, \dodoi{10.1093/mnras/stx1896}

\bibitem[{{Gnat} \& {Sternberg}(2007)}]{GnatSternberg}
{Gnat}, O., \& {Sternberg}, A. 2007, \apjs, 168, 213, \dodoi{10.1086/509786}

\bibitem[{{Goerdt} \& {Ceverino}(2015)}]{GoerdtCeverino2015}
{Goerdt}, T., \& {Ceverino}, D. 2015, \mnras, 450, 3359,
  \dodoi{10.1093/mnras/stv786}

\bibitem[{Goerdt {et~al.}(2010)Goerdt, Read, Moore, \& Stadel}]{Goerdt2010}
Goerdt, T., Read, J.~I., Moore, B., \& Stadel, J. 2010, Astrophys. J., 725,
  1707, \dodoi{10.1088/0004-637X/725/2/1707}

\bibitem[{{Gronke} \& {Oh}(2018)}]{gronke18}
{Gronke}, M., \& {Oh}, S.~P. 2018, \mnras, \dodoi{10.1093/mnrasl/sly131}

\bibitem[{{Gronke} \& {Oh}(2020)}]{gronke20-cloud}
---. 2020, \mnras, 492, 1970, \dodoi{10.1093/mnras/stz3332}

\bibitem[{{Gr{\o}nnow} {et~al.}(2022){Gr{\o}nnow}, {Tepper-Garc{\'\i}a},
  {Bland-Hawthorn}, \& {Fraternali}}]{gronnow22}
{Gr{\o}nnow}, A., {Tepper-Garc{\'\i}a}, T., {Bland-Hawthorn}, J., \&
  {Fraternali}, F. 2022, \mnras, 509, 5756, \dodoi{10.1093/mnras/stab3452}

\bibitem[{{Hennawi} {et~al.}(2015){Hennawi}, {Prochaska}, {Cantalupo}, \&
  {Arrigoni-Battaia}}]{Hennawi2015}
{Hennawi}, J.~F., {Prochaska}, J.~X., {Cantalupo}, S., \& {Arrigoni-Battaia},
  F. 2015, Science, 348, 779, \dodoi{10.1126/science.aaa5397}

\bibitem[{{Hernquist}(1990)}]{Hernquist1990}
{Hernquist}, L. 1990, \apj, 356, 359, \dodoi{10.1086/168845}

\bibitem[{{Hidalgo Pineda} {et~al.}(2023){Hidalgo Pineda}, {Farber}, \&
  {Gronke}}]{hildalgo23}
{Hidalgo Pineda}, F., {Farber}, R.~J., \& {Gronke}, M. 2023, in American
  Astronomical Society Meeting Abstracts, Vol.~55, American Astronomical
  Society Meeting Abstracts, 177.75

\bibitem[{{Hidalgo-Pineda} {et~al.}(2023){Hidalgo-Pineda}, {Farber}, \&
  {Gronke}}]{Pineda2023}
{Hidalgo-Pineda}, F., {Farber}, R.~J., \& {Gronke}, M. 2023, \mnras,
  \dodoi{10.1093/mnras/stad3069}

\bibitem[{{Ji} {et~al.}(2019){Ji}, {Oh}, \& {Masterson}}]{ji19}
{Ji}, S., {Oh}, S.~P., \& {Masterson}, P. 2019, \mnras, 487, 737,
  \dodoi{10.1093/mnras/stz1248}

\bibitem[{{Ji} {et~al.}(2018){Ji}, {Oh}, \& {McCourt}}]{ji18}
{Ji}, S., {Oh}, S.~P., \& {McCourt}, M. 2018, \mnras, 476, 852,
  \dodoi{10.1093/mnras/sty293}

\bibitem[{{Kere{\v{s}}} {et~al.}(2005){Kere{\v{s}}}, {Katz}, {Weinberg}, \&
  {Dav{\'e}}}]{keres05}
{Kere{\v{s}}}, D., {Katz}, N., {Weinberg}, D.~H., \& {Dav{\'e}}, R. 2005,
  \mnras, 363, 2, \dodoi{10.1111/j.1365-2966.2005.09451.x}

\bibitem[{{Klein} {et~al.}(1994){Klein}, {McKee}, \& {Colella}}]{klein94}
{Klein}, R.~I., {McKee}, C.~F., \& {Colella}, P. 1994, \apj, 420, 213,
  \dodoi{10.1086/173554}

\bibitem[{{Kriginsky} {et~al.}(2021){Kriginsky}, {Oliver}, {Antolin},
  {Kuridze}, \& {Freij}}]{kriginsky2021}
{Kriginsky}, M., {Oliver}, R., {Antolin}, P., {Kuridze}, D., \& {Freij}, N.
  2021, \aap, 650, A71, \dodoi{10.1051/0004-6361/202140611}

\bibitem[{{Ledos} {et~al.}(2023){Ledos}, {Takasao}, \&
  {Nagamine}}]{ColdStreamBfield}
{Ledos}, N., {Takasao}, S., \& {Nagamine}, K. 2023, arXiv e-prints,
  arXiv:2308.05412, \dodoi{10.48550/arXiv.2308.05412}

\bibitem[{{Li} {et~al.}(2020{\natexlab{a}}){Li}, {Hopkins}, {Squire}, \&
  {Hummels}}]{Li2020}
{Li}, Z., {Hopkins}, P.~F., {Squire}, J., \& {Hummels}, C. 2020{\natexlab{a}},
  \mnras, 492, 1841, \dodoi{10.1093/mnras/stz3567}

\bibitem[{{Li} {et~al.}(2020{\natexlab{b}}){Li}, {Hopkins}, {Squire}, \&
  {Hummels}}]{li20}
---. 2020{\natexlab{b}}, \mnras, 492, 1841, \dodoi{10.1093/mnras/stz3567}

\bibitem[{{Lim} {et~al.}(2008){Lim}, {Ao}, \& {Dinh-V-Trung}}]{Lim2008}
{Lim}, J., {Ao}, Y., \& {Dinh-V-Trung}. 2008, \apj, 672, 252,
  \dodoi{10.1086/523664}

\bibitem[{{Mandelker} {et~al.}(2020{\natexlab{a}}){Mandelker}, {Nagai}, {Aung},
  {Dekel}, {Birnboim}, \& {van den Bosch}}]{mandelker20}
{Mandelker}, N., {Nagai}, D., {Aung}, H., {et~al.} 2020{\natexlab{a}}, \mnras,
  494, 2641, \dodoi{10.1093/mnras/staa812}

\bibitem[{{Mandelker} {et~al.}(2019{\natexlab{a}}){Mandelker}, {Nagai}, {Aung},
  {Dekel}, {Padnos}, \& {Birnboim}}]{nirkhi2019}
---. 2019{\natexlab{a}}, \mnras, 484, 1100, \dodoi{10.1093/mnras/stz012}

\bibitem[{{Mandelker} {et~al.}(2019{\natexlab{b}}){Mandelker}, {Nagai}, {Aung},
  {Dekel}, {Padnos}, \& {Birnboim}}]{mandelker19}
---. 2019{\natexlab{b}}, \mnras, 484, 1100, \dodoi{10.1093/mnras/stz012}

\bibitem[{{Mandelker} {et~al.}(2016){Mandelker}, {Padnos}, {Dekel}, {Birnboim},
  {Burkert}, {Krumholz}, \& {Steinberg}}]{mandelker16}
{Mandelker}, N., {Padnos}, D., {Dekel}, A., {et~al.} 2016, \mnras, 463, 3921,
  \dodoi{10.1093/mnras/stw2267}

\bibitem[{{Mandelker} {et~al.}(2020{\natexlab{b}}){Mandelker}, {van den Bosch},
  {Nagai}, {Dekel}, {Birnboim}, \& {Aung}}]{mandelker20-blobs}
{Mandelker}, N., {van den Bosch}, F.~C., {Nagai}, D., {et~al.}
  2020{\natexlab{b}}, \mnras, 498, 2415, \dodoi{10.1093/mnras/staa2421}

\bibitem[{{Martin} {et~al.}(2014{\natexlab{a}}){Martin}, {Chang},
  {Matuszewski}, {Morrissey}, {Rahman}, {Moore}, \& {Steidel}}]{Martin2014}
{Martin}, D.~C., {Chang}, D., {Matuszewski}, M., {et~al.} 2014{\natexlab{a}},
  \apj, 786, 106, \dodoi{10.1088/0004-637X/786/2/106}

\bibitem[{{Martin} {et~al.}(2014{\natexlab{b}}){Martin}, {Chang},
  {Matuszewski}, {Morrissey}, {Rahman}, {Moore}, {Steidel}, \&
  {Matsuda}}]{Martin2014b}
---. 2014{\natexlab{b}}, \apj, 786, 107, \dodoi{10.1088/0004-637X/786/2/107}

\bibitem[{{Martin} {et~al.}(2019){Martin}, {O'Sullivan}, {Matuszewski},
  {Hamden}, {Dekel}, {Lapiner}, {Morrissey}, {Neill}, {Cantalupo}, {Prochaska},
  {Steidel}, {Trainor}, {Moore}, {Ceverino}, {Primack}, \&
  {Rizzi}}]{Martin2019}
{Martin}, D.~C., {O'Sullivan}, D., {Matuszewski}, M., {et~al.} 2019, Nature
  Astronomy, 3, 822, \dodoi{10.1038/s41550-019-0791-2}

\bibitem[{{Mart{\'\i}nez-G{\'o}mez} {et~al.}(2020){Mart{\'\i}nez-G{\'o}mez},
  {Oliver}, {Khomenko}, \& {Collados}}]{martinez2020}
{Mart{\'\i}nez-G{\'o}mez}, D., {Oliver}, R., {Khomenko}, E., \& {Collados}, M.
  2020, \aap, 634, A36, \dodoi{10.1051/0004-6361/201937078}

\bibitem[{{Matsuda} {et~al.}(2011){Matsuda}, {Yamada}, {Hayashino}, {Yamauchi},
  {Nakamura}, {Morimoto}, {Ouchi}, {Ono}, {Kousai}, {Nakamura}, {Horie},
  {Fujii}, {Umemura}, \& {Mori}}]{Matsuda2011}
{Matsuda}, Y., {Yamada}, T., {Hayashino}, T., {et~al.} 2011, \mnras, 410, L13,
  \dodoi{10.1111/j.1745-3933.2010.00969.x}

\bibitem[{{McClure-Griffiths} {et~al.}(2010){McClure-Griffiths}, {Madsen},
  {Gaensler}, {McConnell}, \& {Schnitzeler}}]{mcclure10}
{McClure-Griffiths}, N.~M., {Madsen}, G.~J., {Gaensler}, B.~M., {McConnell},
  D., \& {Schnitzeler}, D.~H.~F.~M. 2010, \apj, 725, 275,
  \dodoi{10.1088/0004-637X/725/1/275}

\bibitem[{McCourt {et~al.}(2015)McCourt, O'Leary, Madigan, \&
  Quataert}]{mccourt15}
McCourt, M., O'Leary, R.~M., Madigan, A.-M., \& Quataert, E. 2015, Monthly
  Notices of the Royal Astronomical Society, 449, 2

\bibitem[{{Nelson} {et~al.}(2013){Nelson}, {Vogelsberger}, {Genel}, {Sijacki},
  {Kere{\v{s}}}, {Springel}, \& {Hernquist}}]{Nelson2013}
{Nelson}, D., {Vogelsberger}, M., {Genel}, S., {et~al.} 2013, \mnras, 429,
  3353, \dodoi{10.1093/mnras/sts595}

\bibitem[{{Nelson} {et~al.}(2020){Nelson}, {Sharma}, {Pillepich}, {Springel},
  {Pakmor}, {Weinberger}, {Vogelsberger}, {Marinacci}, \&
  {Hernquist}}]{nelson20}
{Nelson}, D., {Sharma}, P., {Pillepich}, A., {et~al.} 2020, \mnras, 498, 2391,
  \dodoi{10.1093/mnras/staa2419}

\bibitem[{{Padnos} {et~al.}(2018){Padnos}, {Mandelker}, {Birnboim}, {Dekel},
  {Krumholz}, \& {Steinberg}}]{padnos18}
{Padnos}, D., {Mandelker}, N., {Birnboim}, Y., {et~al.} 2018, \mnras, 477,
  3293, \dodoi{10.1093/mnras/sty789}

\bibitem[{{Prochaska} {et~al.}(2014){Prochaska}, {Lau}, \&
  {Hennawi}}]{Prochaska2014}
{Prochaska}, J.~X., {Lau}, M.~W., \& {Hennawi}, J.~F. 2014, \apj, 796, 140,
  \dodoi{10.1088/0004-637X/796/2/140}

\bibitem[{{Prochaska} {et~al.}(2019){Prochaska}, {Macquart}, {McQuinn},
  {Simha}, {Shannon}, {Day}, {Marnoch}, {Ryder}, {Deller}, {Bannister},
  {Bhandari}, {Bordoloi}, {Bunton}, {Cho}, {Flynn}, {Mahony}, {Phillips},
  {Qiu}, \& {Tejos}}]{Prochaska2019}
{Prochaska}, J.~X., {Macquart}, J.-P., {McQuinn}, M., {et~al.} 2019, Science,
  366, 231, \dodoi{10.1126/science.aay0073}

\bibitem[{{Putman} {et~al.}(2012){Putman}, {Peek}, \& {Joung}}]{putman12}
{Putman}, M.~E., {Peek}, J.~E.~G., \& {Joung}, M.~R. 2012, \araa, 50, 491,
  \dodoi{10.1146/annurev-astro-081811-125612}

\bibitem[{{Putman} {et~al.}(2002){Putman}, {de Heij}, {Staveley-Smith},
  {Braun}, {Freeman}, {Gibson}, {Burton}, {Barnes}, {Banks}, {Bhathal}, {de
  Blok}, {Boyce}, {Disney}, {Drinkwater}, {Ekers}, {Henning}, {Jerjen},
  {Kilborn}, {Knezek}, {Koribalski}, {Malin}, {Marquarding}, {Minchin},
  {Mould}, {Oosterloo}, {Price}, {Ryder}, {Sadler}, {Stewart}, {Stootman},
  {Webster}, \& {Wright}}]{putman02}
{Putman}, M.~E., {de Heij}, V., {Staveley-Smith}, L., {et~al.} 2002, \aj, 123,
  873, \dodoi{10.1086/338088}

\bibitem[{{Putman} {et~al.}(2009){Putman}, {Peek}, {Muratov}, {Gnedin}, {Hsu},
  {Douglas}, {Heiles}, {Stanimirovic}, {Korpela}, \& {Gibson}}]{putman09}
{Putman}, M.~E., {Peek}, J.~E.~G., {Muratov}, A., {et~al.} 2009, \apj, 703,
  1486, \dodoi{10.1088/0004-637X/703/2/1486}

\bibitem[{{Ramesh} {et~al.}(2024){Ramesh}, {Nelson}, {Fielding}, \&
  {Br{\"u}ggen}}]{ramesh24}
{Ramesh}, R., {Nelson}, D., {Fielding}, D., \& {Br{\"u}ggen}, M. 2024, \aap,
  684, L16, \dodoi{10.1051/0004-6361/202348786}

\bibitem[{{Roy} {et~al.}(2024){Roy}, {Su}, {Tonnesen}, {Fielding}, \&
  {Faucher-Gigu{\`e}re}}]{roy24}
{Roy}, M., {Su}, K.-Y., {Tonnesen}, S., {Fielding}, D.~B., \&
  {Faucher-Gigu{\`e}re}, C.-A. 2024, \mnras, 527, 265,
  \dodoi{10.1093/mnras/stad3142}

\bibitem[{{Smith} {et~al.}(1990){Smith}, {Heckman}, \&
  {Illingworth}}]{Smith1990}
{Smith}, E.~P., {Heckman}, T.~M., \& {Illingworth}, G.~D. 1990, \apj, 356, 399,
  \dodoi{10.1086/168848}

\bibitem[{{Stone} {et~al.}(2020){Stone}, {Tomida}, {White}, \&
  {Felker}}]{Athena}
{Stone}, J.~M., {Tomida}, K., {White}, C.~J., \& {Felker}, K.~G. 2020, \apjs,
  249, 4, \dodoi{10.3847/1538-4365/ab929b}

\bibitem[{{Tan} \& {Fielding}(2023)}]{TanFielding2023}
{Tan}, B., \& {Fielding}, D.~B. 2023, arXiv e-prints, arXiv:2305.14424,
  \dodoi{10.48550/arXiv.2305.14424}

\bibitem[{{Tan} {et~al.}(2021){Tan}, {Oh}, \& {Gronke}}]{tan21}
{Tan}, B., {Oh}, S.~P., \& {Gronke}, M. 2021, \mnras, 502, 3179,
  \dodoi{10.1093/mnras/stab053}

\bibitem[{{Tan} {et~al.}(2023){Tan}, {Oh}, \& {Gronke}}]{tan23-gravity}
---. 2023, \mnras, 520, 2571, \dodoi{10.1093/mnras/stad236}

\bibitem[{{Tan}(2024)}]{brent25}
{Tan}, Z. Y.~B. 2024, arXiv e-prints, arXiv:2408.10387,
  \dodoi{10.48550/arXiv.2408.10387}

\bibitem[{{Townsend}(2009)}]{Townsend}
{Townsend}, R.~H.~D. 2009, \apjs, 181, 391, \dodoi{10.1088/0067-0049/181/2/391}

\bibitem[{{Tumlinson} {et~al.}(2017){Tumlinson}, {Peeples}, \&
  {Werk}}]{Tumlinson2017}
{Tumlinson}, J., {Peeples}, M.~S., \& {Werk}, J.~K. 2017, \araa, 55, 389,
  \dodoi{10.1146/annurev-astro-091916-055240}

\bibitem[{{Turner} {et~al.}(2017){Turner}, {Schaye}, {Crain}, {Rudie},
  {Steidel}, {Strom}, \& {Theuns}}]{Turner2017}
{Turner}, M.~L., {Schaye}, J., {Crain}, R.~A., {et~al.} 2017, \mnras, 471, 690,
  \dodoi{10.1093/mnras/stx1616}

\bibitem[{{Umehata} {et~al.}(2019){Umehata}, {Fumagalli}, {Smail}, {Matsuda},
  {Swinbank}, {Cantalupo}, {Sykes}, {Ivison}, {Steidel}, {Shapley}, {Vernet},
  {Yamada}, {Tamura}, {Kubo}, {Nakanishi}, {Kajisawa}, {Hatsukade}, \&
  {Kohno}}]{Umehata2019}
{Umehata}, H., {Fumagalli}, M., {Smail}, I., {et~al.} 2019, Science, 366, 97,
  \dodoi{10.1126/science.aaw5949}

\bibitem[{{van de Voort} {et~al.}(2021){van de Voort}, {Bieri}, {Pakmor},
  {G{\'o}mez}, {Grand}, \& {Marinacci}}]{VandeVoort2021}
{van de Voort}, F., {Bieri}, R., {Pakmor}, R., {et~al.} 2021, \mnras, 501,
  4888, \dodoi{10.1093/mnras/staa3938}

\bibitem[{{van de Voort} {et~al.}(2012){van de Voort}, {Schaye}, {Altay}, \&
  {Theuns}}]{Voort2012}
{van de Voort}, F., {Schaye}, J., {Altay}, G., \& {Theuns}, T. 2012, \mnras,
  421, 2809, \dodoi{10.1111/j.1365-2966.2012.20487.x}

\bibitem[{{Veilleux} {et~al.}(2005){Veilleux}, {Cecil}, \&
  {Bland-Hawthorn}}]{Veilleux2005}
{Veilleux}, S., {Cecil}, G., \& {Bland-Hawthorn}, J. 2005, \araa, 43, 769,
  \dodoi{10.1146/annurev.astro.43.072103.150610}

\bibitem[{{Voit} {et~al.}(2019){Voit}, {Donahue}, {Zahedy}, {Chen}, {Werk},
  {Bryan}, \& {O'Shea}}]{voit19}
{Voit}, G.~M., {Donahue}, M., {Zahedy}, F., {et~al.} 2019, \apjl, 879, L1,
  \dodoi{10.3847/2041-8213/ab2766}

\bibitem[{{Yang} \& {Ji}(2023)}]{YangJi2023}
{Yang}, Y., \& {Ji}, S. 2023, \mnras, 520, 2148, \dodoi{10.1093/mnras/stad264}

\bibitem[{{Zabl} {et~al.}(2020){Zabl}, {Bouch{\'e}}, {Schroetter}, {Wendt},
  {Contini}, {Schaye}, {Marino}, {Muzahid}, {Pezzulli}, {Verhamme}, \&
  {Wisotzki}}]{Zabl2020}
{Zabl}, J., {Bouch{\'e}}, N.~F., {Schroetter}, I., {et~al.} 2020, \mnras, 492,
  4576, \dodoi{10.1093/mnras/stz3607}

\bibitem[{{Zhang} {et~al.}(2017){Zhang}, {Thompson}, {Quataert}, \&
  {Murray}}]{zhang17}
{Zhang}, D., {Thompson}, T.~A., {Quataert}, E., \& {Murray}, N. 2017, \mnras,
  468, 4801, \dodoi{10.1093/mnras/stx822}

\bibitem[{{Zhao} \& {Bai}(2023{\natexlab{a}})}]{zhao23}
{Zhao}, X., \& {Bai}, X.-N. 2023{\natexlab{a}}, \mnras,
  \dodoi{10.1093/mnras/stad3011}

\bibitem[{{Zhao} \& {Bai}(2023{\natexlab{b}})}]{TRMLwBfield}
---. 2023{\natexlab{b}}, arXiv e-prints, arXiv:2307.12355,
  \dodoi{10.48550/arXiv.2307.12355}

\end{thebibliography}

